A two-parameter, minimal-data model to predict dengue cases: the 2022-2023 outbreak in Florida, USA

Reliable and timely dengue predictions can provide an actionable lead time for targeted vector control and clinical preparedness, reducing preventable disease and health-system costs in at-risk communities. However, many forecasting approaches depend on site-specific covariates and entomological surveillance, which limits portability to data-sparse settings. In this work, we mathematically prove that a parabolic ICC structure, previously established for the basic SIR model, also holds in a substantially more complex model: a two-population (human-mosquito) four-serotype dengue transmission model with primary and secondary infections and mild/severe disease classes. To predict the number of new cases, we propose a data-parsimonious (DP) framework built on the incidence-cumulative cases (ICC) curve that requires only the human incidence time series of the target season and estimates only two parameters, thereby reducing estimation noise and computational burden. We further develop a Bayesian extension that accounts for case-reporting and fitting uncertainty, producing calibrated predictive intervals. The Bayesian model yields improved predictive performance compared to the parabolic ICC model. We evaluate the framework for dengue outbreaks in Florida in 2022-2023, where standardized clinical tests and reporting support accurate case determination.

==> makefile <==
# $Id: makefile 282 2026-01-08 05:54:22Z rishi $

file=elsdoc


all: pdf out 
	make pdf
	make pdf

#out:
#	if  [ -f $(file).out ] ; then cp $(file).out tmp.out; fi ;
#	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ;

out:
	if  [ -f "$(file).out" ] ; then cp "$(file).out" tmp.out; fi ; 
	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ; 
	sed -i 's/{\\376\\377/{/g' tmp.out ; 
	sed -i '/dtxmark/s/\\000//g' tmp.out
	sed -i 's/\\040/ /g' tmp.out ; 
	sed -i 's/\t/ /g' tmp.out

pdf:
	pdflatex $(file).tex

index:
	makeindex -s gind.ist -o $(file).ind $(file).idx 

changes:
	makeindex -s gglo.ist -o $(file).gls $(file).glo

xview:
#	xpdf -z 200 $(file).pdf &>/dev/null
	open -a 'Skim.app' $(file).pdf 

view:
	open -a 'Adobe Reader.app' $(file).pdf

ins:
	latex $(file).ins 

diff:
	diff $(file).sty ../$(file).sty |less

copy:
	cp $(file).sty ../


